CoViS-Net: A Cooperative Visual Spatial Foundation Model for Multi-Robot Applications

Autonomous robot operation in unstructured environments is often underpinned by spatial understanding through vision. Systems composed of multiple concurrently operating robots additionally require access to frequent, accurate and reliable pose estimates. In this work, we propose CoViS-Net, a decentralized visual spatial foundation model that learns spatial priors from data, enabling pose estimation as well as spatial comprehension. Our model is fully decentralized, platform-agnostic, executable in real-time using onboard compute, and does not require existing networking infrastructure. CoViS-Net provides relative pose estimates and a local bird's-eye-view (BEV) representation, even without camera overlap between robots (in contrast to classical methods). We demonstrate its use in a multi-robot formation control task across various real-world settings. We provide code, models and supplementary material online. https://proroklab.github.io/CoViS-Net/

==> figs/architecture/architecture_vertical.tex <==
\begin{tikzpicture}[auto,>=latex']
    \tikzset{
        enc/.style = {minimum width=1.5cm, minimum height=1.9em, trapezium, trapezium angle=-75, draw, trapezium stretches=true, inner sep=0.4em},
        node_label/.style = {inner sep=0.4em},
        block/.style = {draw=black, inner sep=0.4em},
        colored/.style = {fill=orange!30},
        img/.style = {inner sep=0pt},
        comm/.style = {decorate,decoration={snake, amplitude=0.4mm, segment length=3mm, post length=1mm}},
    }
    
    % nodes
    %% img/enc i
    \node[img] (img_i) {\includegraphics[width=1.5cm]{figs/architecture/img_25_0.jpg}};
    \node [enc, colored, below=1.5em of img_i, transform shape] (f_enc_i) {$\fenc$};

    %% img/enc j
    \node[img, right=1.75cm of img_i] (img_j) {\includegraphics[width=1.5cm]{figs/architecture/img_25_1.jpg}};
    \node [enc, colored, below=1.5em of img_j, transform shape] (f_enc_j) {$\fenc$};

    %% img/enc k
    \node[img, left=1.75cm of img_i] (img_k) {\includegraphics[width=1.5cm]{figs/architecture/img_25_2.jpg}};
    \node [enc, colored, below=1.5em of img_k, transform shape] (f_enc_k) {$\fenc$};

    %% Pose nodes
    \node [block, colored, below=3em of $(f_enc_i.south)!0.5!(f_enc_j.south)$] (pose_ij) {$\fpose$};
    \node [above=0.75em of pose_ij] (pose_ij_pred) {$\posest{i}{ij}, \rotest{i}{ij}, \edgeu{ij}$};

    \node [block, colored, below=3em of $(f_enc_i.south)!0.5!(f_enc_k.south)$] (pose_ik) {$\fpose$};
    \node [above=0.75em of pose_ik] (pose_ik_pred) {$\posest{i}{ik}, \rotest{i}{ik}, \edgeu{ik}$};

    %% cat nides
    \node [circle, draw, inner sep=1pt, below=1.5em of pose_ij] (pose_ij_cat) {$\vert\vert_{F}$};
    \node [circle, draw, inner sep=1pt, below=1.5em of pose_ik] (pose_ik_cat) {$\vert\vert_{F}$};
    \node [circle, draw, inner sep=1pt] (pose_ii_cat) at ($(pose_ik_cat.east)!0.5!(pose_ij_cat.west)$) {$\vert\vert_{F}$};

    \node [block, colored, below=2.5em of pose_ii_cat] (f_agg) {$\fagg$};
    \node [right=1.0em of f_agg] (f_agg_out) {$\nodeemb{i}$};

    \node [left=0.5em of pose_ii_cat] (pose_ii_zero) {$\mathbf{0}$};
    \node [coordinate] (f_agg_emb) at ($(pose_ii_cat)!0.6!(f_agg)$) {$\vert\vert_{F}$};


    % connectors
    \draw[->](img_i.south) -- node[node_label, pos=0.5,right] {$\img{i}$} (f_enc_i.north);
    \draw[->](img_k.south) -- node[node_label, pos=0.5,right] {$\img{k}$} (f_enc_k.north);
    \draw[->](img_j.south) -- node[node_label, pos=0.5,right] {$\img{j}$} (f_enc_j.north);

    \draw[->](f_enc_k.south) |- node[pos=0.1,left] {$\imgemb{k}$} (pose_ik.west);
    \draw[->](f_enc_k.south) |- (pose_ik_cat.west);
    
    \draw[->](f_enc_j.south) |- node[pos=0.1,right] {$\imgemb{j}$} (pose_ij.east);
    \draw[->](f_enc_j.south) |- (pose_ij_cat.east);
    
    \draw[->](f_enc_i.south) -- node[pos=0.5,right] {$\imgemb{i}$} (pose_ii_cat.north);
    \draw[->](f_enc_i.south) |- (pose_ij.west);
    \draw[->](f_enc_i.south) |- (pose_ik.east);

    \draw[->](pose_ij.north) -- (pose_ij_pred);
    \draw[->](pose_ik.north) -- (pose_ik_pred);
    \draw[->](pose_ik.south) -- node[pos=0.5,left] {$\imgemb{ik}$} (pose_ik_cat.north);
    \draw[->](pose_ij.south) -- node[pos=0.5,right] {$\imgemb{ij}$} (pose_ij_cat.north);

    \draw[->](pose_ii_zero.east) -- (pose_ii_cat);

    \draw[->](pose_ik_cat.south) |- node[pos=0.3,left] {$\nodeemb{ik}$} (f_agg_emb) -- (f_agg.north);
    \draw[->](pose_ij_cat.south) |- node[pos=0.3,right] {$\nodeemb{ij}$} (f_agg_emb) -- (f_agg.north);
    \draw[-](pose_ii_cat.south) |- node[pos=0.3,right] {$\nodeemb{ii}$} (f_agg_emb);

    \draw[->](f_agg.east) -- (f_agg_out);
\end{tikzpicture}


==> figs/tables/table_run_ablation_real.tex <==
256 & 48 & 24 kB & $\mathbf{67}$ \textbf{cm, }$\mathbf{14.1^\circ}$ & $47$ cm, $6.4^\circ$ & $\mathbf{107}$ \textbf{cm, }$\mathbf{19.4^\circ}$ & $\mathbf{97}$ \textbf{cm, }$\mathbf{7.9^\circ}$ & $48$ cm, $11.6^\circ$ & $33$ cm, $5.8^\circ$ \\
128 & 96 & 24 kB & $68$ cm, $12.6^\circ$ & $46$ cm, $6.1^\circ$ & $114$ cm, $18.6^\circ$ & $97$ cm, $7.4^\circ$ & $47$ cm, $9.7^\circ$ & $32$ cm, $5.6^\circ$ \\
128 & 48 & 12 kB & $74$ cm, $18.1^\circ$ & $\mathbf{45}$ \textbf{cm, }$\mathbf{6.6^\circ}$ & $132$ cm, $34.9^\circ$ & $113$ cm, $9.6^\circ$ & $\mathbf{47}$ \textbf{cm, }$\mathbf{10.2^\circ}$ & $\mathbf{29}$ \textbf{cm, }$\mathbf{5.7^\circ}$ \\
128 & 24 & 6 kB & $75$ cm, $16.8^\circ$ & $46$ cm, $6.7^\circ$ & $132$ cm, $30.6^\circ$ & $112$ cm, $9.7^\circ$ & $47$ cm, $10.3^\circ$ & $31$ cm, $5.7^\circ$ \\
64 & 48 & 6 kB & $82$ cm, $21.8^\circ$ & $54$ cm, $7.3^\circ$ & $136$ cm, $39.1^\circ$ & $119$ cm, $10.8^\circ$ & $56$ cm, $13.7^\circ$ & $36$ cm, $6.3^\circ$ \\
\midrule
1 & 3072 & 6 kB & $104$ cm, $97.8^\circ$ & $102$ cm, $105.0^\circ$ & $119$ cm, $27.3^\circ$ & $122$ cm, $25.8^\circ$ & $97$ cm, $131.1^\circ$ & $93$ cm, $138.2^\circ$ \\
1 & 348 & 696 B & $114$ cm, $41.2^\circ$ & $98$ cm, $14.7^\circ$ & $147$ cm, $68.7^\circ$ & $135$ cm, $37.9^\circ$ & $99$ cm, $28.3^\circ$ & $80$ cm, $11.1^\circ$ \\


==> figs/tables/table_run_ablation_sim.tex <==
256 & 48 & 24 kB & $\mathbf{0.571}$ & $\mathbf{0.691}$ & $78$ cm, $25.1^\circ$ & $\mathbf{36}$ \textbf{cm, }$\mathbf{8.3^\circ}$ \\
128 & 96 & 24 kB & $0.568$ & $0.688$ & $81$ cm, $26.0^\circ$ & $40$ cm, $8.4^\circ$ \\
128 & 48 & 12 kB & $0.561$ & $0.679$ & $\mathbf{75}$ \textbf{cm, }$\mathbf{21.2^\circ}$ & $38$ cm, $7.7^\circ$ \\
128 & 24 & 6 kB & $0.546$ & $0.667$ & $89$ cm, $30.2^\circ$ & $50$ cm, $9.5^\circ$ \\
64 & 48 & 6 kB & $0.435$ & $0.610$ & $91$ cm, $29.9^\circ$ & $51$ cm, $9.6^\circ$ \\
\midrule
1 & 3072 & 6 kB & $0.014$ & $0.470$ & $151$ cm, $90.3^\circ$ & $144$ cm, $89.9^\circ$ \\
1 & 348 & 696 B & $0.014$ & $0.471$ & $111$ cm, $33.8^\circ$ & $84$ cm, $11.7^\circ$ \\


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
